Effectiveness of Tree-based Ensembles for Anomaly Discovery: Insights, Batch and Streaming Active Learning

In many real-world AD applications including computer security and fraud prevention, the anomaly detector must be configurable by the human analyst to minimize the effort on false positives. One important way to configure the detector is by providing true labels (nominal or anomaly) for a few instances. Recent work on active anomaly discovery has shown that greedily querying the top-scoring instance and tuning the weights of ensemble detectors based on label feedback allows us to quickly discover true anomalies. This paper makes four main contributions to improve the state-of-the-art in anomaly discovery using tree-based ensembles. First, we provide an important insight that explains the practical successes of unsupervised tree-based ensembles and active learning based on greedy query selection strategy. We also present empirical results on real-world data to support our insights and theoretical analysis to support active learning. Second, we develop a novel batch active learning algorithm to improve the diversity of discovered anomalies based on a formalism called compact description to describe the discovered anomalies. Third, we develop a novel active learning algorithm to handle streaming data setting. We present a data drift detection algorithm that not only detects the drift robustly, but also allows us to take corrective actions to adapt the anomaly detector in a principled manner. Fourth, we present extensive experiments to evaluate our insights and our tree-based active anomaly discovery algorithms in both batch and streaming data settings. Our results show that active learning allows us to discover significantly more anomalies than state-of-the-art unsupervised baselines, our batch active learning algorithm discovers diverse anomalies, and our algorithms under the streaming-data setup are competitive with the batch setup.

==> algorithm_glad.tex <==
\section{Active Learning Algorithms for Generic Ensembles}
\label{sec:glad}

In this section, we first describe an active anomaly detection algorithm referred as GLAD that is applicable to generic (homogeneous or heterogeneous) ensemble of detectors. Subsequently, we describe a GLAD-specific approach to generate succinct explanations to help the human analyst.

\vspace{-1.0ex}

\subsection{GLocalized Anomaly Detection via Active Feature Space Suppression}

\paragraph{Definition 1 (\textit{Glocal})}  \textit{Reflecting or characterized by both local and global considerations\footnote{\url{https://en.wikipedia.org/wiki/Glocal} (retrieved on 29-Dec-2018)}.}

\vspace{1.0ex}

A majority of the active learning techniques for discovering anomalies, including those presented above, employ a weighted linear combination of the anomaly scores from the ensemble members. This approach works well when the ensemble contains a large number of members which are themselves highly localized, such as the leaf nodes of tree-based detectors. However, when there are a {\em small} number of detectors in the ensemble and/or the members of the ensemble are global (such as LODA projections \cite{pevny:2015}), it is highly likely that individual detectors are incorrect in at least some local parts of the input feature space. To overcome this drawback,  we propose a principled technique --- {\em GLocalized Anomaly Detection (GLAD)} --- which allows a human analyst to continue using anomaly detection ensembles with global behavior by learning their local relevance in different parts of the feature space via label feedback. Our GLAD algorithm automatically learns the {\em local relevance} of each ensemble member in the feature space via a neural network using the label feedback from a human analyst.

Our GLAD technique is similar in spirit to dynamic ensemble weighting \cite{jimenez:1998}. However, since we are in an active learning setting for anomaly detection, we need to consider two important aspects: {\bf (a)} Number of labeled examples is very small (possibly none), and {\bf (b)} To reduce the effort of the human analyst, the algorithm needs to be \textit{primed} so that the likelihood of discovering anomalies is very high from the first feedback iteration itself. 

\vspace{2.0ex}

\noindent {\bf Overview of GLAD Algorithm.} We assume the availability of an ensemble $\mathcal{E}$ of $M$ (global) anomaly detectors (e.g., LODA projections) which assign scores $s_1({\bf x}), s_2({\bf x}),\cdots, s_M({\bf x})$ to each instance ${\bf x} \in \mathcal{X}$. Suppose that $p_m({\bf x}) \in [0, 1]$ denotes the relevance of the $m^{th}$ ensemble member  for a data instance ${\bf x}$. We employ a neural network to predict the local relevance of each ensemble member. The scores of $M$ anomaly detectors are combined as follows: \texttt{Score}(${\bf x}$) = $\sum_{m=1}^M{s_m({\bf x}) \cdot p_m({\bf x})}$. We incorporate the insights discussed in Section~\ref{sec:insights} for GLAD as follows. We start with the assumption that each ensemble member is uniformly relevant in every part of the input feature space. This assumption is implemented by priming a neural network referred to as \textit{FSSN} (feature space suppression network) with parameters ${\bf \Theta}$ to predict the same probability value $b \in (0, 1)$ for every instance in ${\bf D}$. In effect, this mechanism places \textit{\textbf{a uniform prior over the input feature space $\mathcal{X}$} for the relevance of each detector}. Subsequently, the algorithm receives label feedback from a human analyst and determines whether the ensemble made an error (i.e., anomalous instances are ranked at the top and scores of anomalies are higher than scores of nominals). If there was an error, the weights of FSSN are updated to suppress all erroneous detectors for similar inputs in the future. Figure~\ref{fig:architecture} illustrates the different components of the GLAD algorithm (Algorithm~\ref{alg:glad}) including the ensemble of anomaly detectors and the FSSN.

\begin{figure}
	\centering
	\subfloat{\includegraphics[width=1.0\textwidth]{figures/AFSS}}
	\caption{Overview of GLAD Algorithm. In each iteration, we select one unlabeled instance for querying, and update the weights of FSSN to adjust the local relevance of each ensemble member over all labeled instances.}
	\label{fig:architecture}
\end{figure}

\vspace{2.0ex}

\paragraph{Loss Function.} We employ a hinge loss similar to that in Equation~\ref{eqn:aatploss}, but tailored to the GLAD-specific score. We will denote this loss by $\ell_{AAD}({\bf x})$ (Equation~\ref{eqn:aad_loss}).

\vspace{-3.0ex}
\begin{align}
\ell_{prior}({\bf x}) &= \sum_{m=1}^M{-b\log(p_m({\bf x})) -(1 - b)\log(1 - p_m({\bf x}))} \label{eqn:prior} \\
\ell_A(q; ({\bf x}, y)) &= \max(0, y (q - \text{\texttt{Score}$({\bf x})$})) \label{eqn:la_loss} \\
\ell_{AAD}({\bf x}, y) &= \ell_A(q_{\tau}^{(t-1)}; ({\bf x}, y)) + \ell_A(\text{\texttt{Score}}({\bf x}_{\tau}^{(t-1)}); ({\bf x}, y)) \label{eqn:aad_loss} \\
\ell_{FSSN} &= \frac{1}{|{\bf H}_f^{(t)}|} \sum_{({\bf x}, y) \in {\bf H}_f^{(t)}} \ell_{AAD}({\bf x}, y) + \frac{\lambda}{|{\bf D}|} \sum_{{\bf x} \in {\bf D}}\ell_{prior}({\bf x}) \label{eqn:loss_fssn}
\end{align}

\vspace{2.0ex}

\paragraph{Feature Space Suppression Network (FSSN).} The FSSN is a neural network with $M$ sigmoid activation nodes in its output layer, where each output node is paired with an ensemble member. It takes as input an instance from the original feature space and outputs the relevance of each detector for that instance. We denote the relevance of the $m^{th}$ detector to instance ${\bf x}$ by $p_m({\bf x})$. The FSSN is primed using the cross-entropy loss in Equation~\ref{eqn:prior} such that it outputs the same probability $b \in (0, 1)$ at all the output nodes for each data instance in ${\bf D}$. This loss acts as a prior on the relevance of detectors in ensemble. When all detectors have the same relevance, the final anomaly score simply corresponds to the average score across all detectors (up to a multiplicative constant), and is \textbf{a good starting point for active learning.} The FSSN must have sufficient capacity to be able to learn to output the same value for every instance non-trivially. This is not hard with neural networks as the capacity can be increased simply by adding a few more hidden nodes. For improved robustness and generalization, it is preferable to select the simplest network that can achieve this goal.

After FSSN is primed, it automatically learns the relevance of the detectors based on label feedback from human analyst using the combined loss $\ell_{FSSN}$ in Equation~\ref{eqn:loss_fssn}, where $\lambda$ is the trade-off parameter. We set the value of $\lambda$ to 1 in all our experiments. $\mathbf{H}_f^{(t)} \subseteq {\bf D}$ in Equation~\ref{eqn:loss_fssn} denotes the total set of instances labeled by the analyst after $t$ feedback iterations. ${\mathbf x}_{\tau}^{(t-1)}$ and $q_{\tau}^{(t-1)}$ denote the instance ranked at the $\tau$-th quantile and its score after the $(t-1)$-th feedback iteration. $\ell_{A}$ encourages the scores of anomalies in $\mathbf{H}_f$ to be higher than that of $q$, and the scores of nominals in $\mathbf{H}_f$ to be lower.

\begin{algorithm}
	%\footnotesize
	\caption{\texttt{GLAD} ($B$, $\mathcal{E}$, {\em FSSN}, ${\mathbf D}$, ${\mathbf H}_f$, $b$)}
	\label{alg:glad}
	\begin{algorithmic}
		\STATE \textbf{Input:} Query budget $B$, Ensemble $\mathcal{E}$,
		\STATE \hspace{0.1in} Feature Space Suppression Network {\em FSSN} with parameters ${\bf \Theta}$,
		\STATE \hspace{0.1in} complete dataset ${\mathbf D}$, labeled instances ${\mathbf H}_f \subseteq {\bf D}$, bias probability $b$
		\STATE Initialize {\em FSSN} to predict $b$ for all ${\bf x} \in {\bf D}$ // priming step
		\FOR{$t \in \{1 \cdots B\}$}
		\STATE
		\STATE // get the vector of anomaly scores for unlabeled instances
		\STATE Set ${\mathbf a}$ = \texttt{Score}(${\mathbf D} \setminus \{x: (x, .) \in {\bf H}_f\}$, $\mathcal{E}$, {\em FSSN})
		\STATE
		\STATE // greedy query strategy: label most anomalous instance
		\STATE Let ${\bf q} = {\mathbf x}_i$, where $i = \argmax_{i}(a_i)$
		\STATE Get label $y_i \in \{-1,+1\}$ for ${\mathbf q}$ from human analyst
		\STATE Set ${\mathbf H}_f = \{({\bf x}_i, y_i)\} \cup {\mathbf H}_f$
		\STATE
		\STATE Update the parameters of {\em FSSN} by minimizing loss in Equation~\ref{eqn:loss_fssn} \label{alg:glad:update}
		\STATE
		\ENDFOR
		\RETURN {\em FSSN}, ${\mathbf H}_f$
	\end{algorithmic}
\end{algorithm}

\paragraph{Illustration of GLAD on {\em Toy} Data.} We employed a shallow neural network with $50$ hidden nodes as the FSSN. The anomaly detection ensemble comprises of the four LODA projections shown in Figure~\ref{fig:dataset}. Figure~\ref{fig:loda_scores} illustrates the aspect that detectors are varying in quality. Figure~\ref{fig:loda_relevance} shows that GLAD learns useful relevance information that can be of help to the analyst.

\begin{figure}
	\centering
	\subfloat[Baseline LODA score contours]{\includegraphics[width=0.48\textwidth]{contours/test_afss_toy2_loda_4w} \label{fig:loda_all}} 
	\subfloat[Score contours for each LODA projection]{\includegraphics[width=0.48\textwidth]{contours/test_loda_toy2_active_4w_ensemble} \label{fig:loda_scores}} \\
	%\subfloat[Initial uniform relevance ($b=0.5$)]{\includegraphics[width=0.48\textwidth]{contours/test_afss_toy2_active_4w_before} \label{fig:loda_uniform}} 
	\subfloat[Learned scores after 30 iterations]{\includegraphics[width=0.48\textwidth]{contours/test_afss_toy2_anomaly_scores_4w_feedback_after} \label{fig:learned_scores}} 
	\subfloat[Relevance after 30 feedback iterations]{\includegraphics[width=0.48\textwidth]{contours/test_afss_toy2_active_4w_f30_after} \label{fig:loda_relevance}}
	\caption{\textit{Toy} data. More red on the \textbf{top row} indicates more \textit{anomalous}. More red on the \textbf{bottom row} indicates more \textit{relevant}. The red `$\times$' are true anomalies and grey `$\times$' are true nominals. {\bf (a)} LODA with four projections (green lines) applied to the \textit{Toy} dataset. {\bf (b)} The contours of only the \textit{bottom left} LODA projection are somewhat aligned with the true anomalies, i.e., most anomalies lie in the higher anomaly score regions. Other projections are highly inaccurate. {\bf (c)} The learned anomaly scores output by GLAD after 30 feedback iterations. {\bf (d)} The points circled in green were shown to the analyst for labeling, one per feedback iteration. After $30$ feedback iterations, the bottom left projection was found to be most relevant in the top-right half-space, whereas it is completely irrelevant in the bottom-left half-space. Other projections were less relevant in most parts of the feature space.}
	\label{fig:dataset}
\end{figure}

\vspace{2.0ex}

\noindent {\bf GLAD vs. Tree-based AAD.} We may consider GLAD as very similar to the Tree-based AAD approach. Tree-based AAD method partitions the input feature space into discrete subspaces and then places a uniform prior over those subspaces (i.e., the uniform weight vector to combine ensemble scores). If we take this view to an extreme by imagining that each instance in the feature space represents a subspace, we can see the connection to GLAD. While Tree-based AAD assigns the scores of discrete subspaces to instances (e.g., node depths for Isolation Forest), the scores assigned by GLAD are continuous, defined by the global ensemble members. The {\em relevance} in GLAD is analogous to the {\em learned weights} in Tree-based AAD. This similarity lets us extend the key insight behind active learning with tree-based models (Section~\ref{sec:insights}) to GLAD as well: uniform prior over weights of each subspace (leaf node) in Tree-based AAD and uniform prior over input feature space for the relevance of each ensemble member in GLAD are highly beneficial for label-efficient active learning. On the basis of this argument and its supporting empirical evidence, we claim that the following hypothesis is true:

\vspace{2.0ex}

\parbox{14.0cm}{\em{Under an uniform prior on the detectors' relevance over the input space, the greedy query selection strategy is label-efficient for active learning with any ensemble of {\bf pre-trained} anomaly detectors.}}

\vspace{2.0ex}

\noindent {\bf Broader Applicability of the Key Idea behind GLAD.} In practice, we often do not have control over the ensemble members. For example, the ensemble might have only a limited number of detectors. In the extreme case, there might only be a single pre-trained detector which cannot be modified. A scoring model that combines detector scores linearly would then lack capacity if the number of labeled instances (obtained through feedback) is high. In this case, GLAD can increase the capacity for incorporating feedback through the FSSN. The FSSN allows us to place a uniform prior over the input space. This property can be employed for domain adaptation of not only anomaly detector ensembles, but also other algorithms including classifier ensembles {\em after they are deployed}.

GLAD employs the AAD loss (Equation~\ref{eqn:aad_loss}) for ranking scores relative to $q_{\tau}$ and ${\bf x}_{\tau}$ in a more general manner when compared to the linear scoring function. This technique can be applied more generally to {\em any} parameterized non-ensemble detector as well (such as the one based on density estimation) for both semi-supervised and active learning settings.

\subsection{Explanations for Anomalies with GLAD}

To help the analyst understand the results of active anomaly detection system, we have used the concept of ``descriptions'' for the tree-based ensembles. We now introduce the concept of ``explanations'' in the context of GLAD algorithm. While both descriptions and explanations seem similar, they are actually quite different:

\begin{itemize}
	\item \textbf{Description:} A description generates a compact representation for a group of instances. The main application is to reduce the cognitive burden on the analysts while providing labeling feedback for queried instances.
	\item \textbf{Explanation:} An explanation outputs a reason why a specific data instance was assigned a high anomaly score. Generally, we limit the scope of an explanation to one data instance. The main application is to diagnose the model: whether the anomaly detector(s) are working as expected or not.
\end{itemize}

GLAD assumes that the anomaly detectors in the ensemble can be arbitrary (homogeneous or heterogeneous). The best it can offer as an explanation is to output the member which is most relevant for a test data instance. With this in mind, we can employ the following approach to generate explanations:

\begin{enumerate}

	\item Employ the FSSN network to predict the relevance of individual ensemble members on the complete dataset. It is important to note that the relevance of a detector is different from the anomaly score(s) it assigns. A detector which is relevant in a particular subspace predicts the labels of instances in that subspace correctly irrespective of whether those instances are anomalies or nominals.
	
	\item Find the instances for each ensemble member for which that detector is the most relevant. Mark these instances as positive and the rest as negative.
	
	\item Train a separate decision tree for each member to separate the corresponding positives and negatives. This describes the subspaces where each ensemble member is relevant. Figure~\ref{fig:glad_relevance} illustrates this idea on the {\em Toy} dataset.
	
	\item When asked to explain the anomaly score for a given test instance:
	
	\begin{enumerate}
		\item Use FSSN network to identify the most relevant ensemble member for the test instance.
		\item Employ a model agnostic explanation technique such as LIME \cite{ribeiro:2016} or ANCHOR \cite{ribeiro:2018} to generate the explanation using the most relevant ensemble member. As a simple illustration, we trained GLAD on the synthetic dataset and a LODA ensemble with four projections. After $30$ feedback iterations, the unlabeled instance at $(6.12, 3.04)$ had the highest anomaly score. We used LIME to explain its anomaly score. LIME explanation is shown below:
		\begin{verbatim}
		('2.16 < y <= 3.31', -0.4253860500153764)
		('x > 2.65', 0.3406543313093905)
		\end{verbatim}
		Here the explanation \texttt{2.16 < y <= 3.31} from member $2$ has the highest absolute weight and hence, explains most of the anomaly score.
	\end{enumerate}
\end{enumerate}

Since most aspects of explanations are qualitative, we leave their evaluation on real-world data to future work.

\begin{figure}
	\centering
	\subfloat{\includegraphics[width=1.0\textwidth]{explanations/test_afss_toy2_active_4wrel_regions_r1}}
	\caption{Most relevant ensemble members in subspaces inferred with GLAD after 30 feedback iterations. There are four members (i.e., LODA projections) in our current example. The region where a member is ranked as the top-most relevant detector is shown in red. Note that members 0 and 1 were found relevant in subspaces which have mostly nominal instances. This is because they correctly assigned low anomaly scores to instances in those subspaces. The last member (member 3) did not rank as the top-most relevant detector for any instance; hence, it does not have any region marked in red. The point circled in green (in bottom left plot) is a test instance. Ensemble member 2 was found to be the most relevant for this instance.}
	\label{fig:glad_relevance}
\end{figure}

